xNeuSM: Explainable Neural Subgraph Matching with Graph Learnable Multi-hop Attention Networks

Subgraph matching is a challenging problem with a wide range of applications in database systems, biochemistry, and cognitive science. It involves determining whether a given query graph is present within a larger target graph. Traditional graph-matching algorithms provide precise results but face challenges in large graph instances due to the NP-complete problem, limiting their practical applicability. In contrast, recent neural network-based approximations offer more scalable solutions, but often lack interpretable node correspondences. To address these limitations, this article presents xNeuSM: Explainable Neural Subgraph Matching which introduces Graph Learnable Multi-hop Attention Networks (GLeMA) that adaptively learns the parameters governing the attention factor decay for each node across hops rather than relying on fixed hyperparameters. We provide a theoretical analysis establishing error bounds for GLeMA's approximation of multi-hop attention as a function of the number of hops. Additionally, we prove that learning distinct attention decay factors for each node leads to a correct approximation of multi-hop attention. Empirical evaluation on real-world datasets shows that xNeuSM achieves substantial improvements in prediction accuracy of up to 34% compared to approximate baselines and, notably, at least a seven-fold faster query time than exact algorithms. The source code of our implementation is available at https://github.com/martinakaduc/xNeuSM.

==> sections/exp_sensitivity.tex <==
\subsection{Hyper-parameter Sensitivity}

\autoref{fig:sensitivity}

\begin{figure}[!h]
    \vspace{-0.3cm}
  \centering
  \includegraphics[width=0.8\linewidth]{images/sensitivity.png}
  \vspace{-0.2cm}
  \caption{Parameter sensitive analysis.}
  \label{fig:sensitivity}
  \vspace{-0.5cm}
\end{figure}
